4DGS-CC: A Contextual Coding Framework for 4D Gaussian Splatting Data Compression

Storage is a significant challenge in reconstructing dynamic scenes with 4D Gaussian Splatting (4DGS) data. In this work, we introduce 4DGS-CC, a contextual coding framework that compresses 4DGS data to meet specific storage constraints. Building upon the established deformable 3D Gaussian Splatting (3DGS) method, our approach decomposes 4DGS data into 4D neural voxels and a canonical 3DGS component, which are then compressed using Neural Voxel Contextual Coding (NVCC) and Vector Quantization Contextual Coding (VQCC), respectively. Specifically, we first decompose the 4D neural voxels into distinct quantized features by separating the temporal and spatial dimensions. To losslessly compress each quantized feature, we leverage the previously compressed features from the temporal and spatial dimensions as priors and apply NVCC to generate the spatiotemporal context for contextual coding. Next, we employ a codebook to store spherical harmonics information from canonical 3DGS as quantized vectors, which are then losslessly compressed by using VQCC with the auxiliary learned hyperpriors for contextual coding, thereby reducing redundancy within the codebook. By integrating NVCC and VQCC, our contextual coding framework, 4DGS-CC, enables multi-rate 4DGS data compression tailored to specific storage requirements. Extensive experiments on three 4DGS data compression benchmarks demonstrate that our method achieves an average storage reduction of approximately 12 times while maintaining rendering fidelity compared to our baseline 4DGS approach.

==> ICCV2025-Author-Kit/1_Abstract.tex <==
\begin{abstract}

% 4D Gaussian Splatting (4DGS) is a promising emerging technology that enables real-time reconstruction and rendering of dynamic scenes with high fidelity. However, it presents significant challenges in data storage and transmission, as a short video of a real-world scene requires tens of megabytes of storage. 
%
% To achieve a highly compact 4DGS representation, we propose 4DGS-CC, which utilizes contexture coding to reduce the primary redundancy in 4DGS.
% Our primary objective is to minimize redundancy in the spatiotemporal structure encoder used to encode the transformation of the scene with time, occupies a substantial portion of the storage. We introduce Deformation field Contexture Coding (DCC), an autoregressive context model combined with both level-wise and neighbor-wise context models to capture spatiotemporal dependencies. This enables probability prediction for information entropy reduction.
% To further reduce redundancy in the Gaussian attributes, specifically the spherical harmonics, we propose Vector Quantization Contexture Coding (VCC). After significantly reducing the number of spherical harmonics through traditional vector quantization, we employ a low-dimensional latent to predict the distribution of high-dimensional codes, facilitating efficient entropy encoding.
% Experimental results show that, compared to the original 4DGS, our framework reduces storage space by approximately 12× across multiple datasets while maintaining visual quality. Only about 4 MB is required to reconstruct a real-world dynamic scene using 4DGS-CC.
\vspace{-3mm}

Storage is a significant challenge in reconstructing dynamic scenes with 4D Gaussian Splatting (4DGS) data. In this work, we introduce 4DGS-CC, a contextual coding framework that compresses 4DGS data to meet specific storage constraints.
%
Building upon the established deformable 3D Gaussian Splatting (3DGS) method, our approach decomposes 4DGS data into 4D neural voxels and a canonical 3DGS component, which are then compressed using Neural Voxel Contextual Coding (NVCC) and Vector Quantization Contextual Coding (VQCC), respectively.
%
Specifically, we first decompose the 4D neural voxels into distinct quantized features by separating the temporal and spatial dimensions. To losslessly compress each quantized feature, we leverage the previously compressed features from the temporal and spatial dimensions as priors and apply NVCC to generate the spatiotemporal context for contextual coding.
%
Next, we employ a codebook to store spherical harmonics information from canonical 3DGS as quantized vectors, which are then losslessly compressed by using VQCC with the auxiliary learned hyperpriors for contextual coding, thereby reducing redundancy within the codebook.
%
By integrating NVCC and VQCC, our contextual coding framework, 4DGS-CC, enables multi-rate 4DGS data compression tailored to specific storage requirements. Extensive experiments on three 4DGS data compression benchmarks demonstrate that our method achieves an average storage reduction of approximately \textbf{12$\times$} while maintaining rendering fidelity compared to our baseline 4DGS approach.
%


% By further incorporating commonly used quantization methods and opacity regulation techniques,our framework achieves a storage reduction by approximately 12× compared to the original 4DGS on multiple datasets while maintaining visual quality.
\end{abstract}

% 1. 4D Gaussian Splatting for Real-Time Dynamic Scene Rendering https://arxiv.org/abs/2310.08528
% 2. 4D Gaussian Splatting with Scale-aware Residual Field and Adaptive Optimization for Real-time Rendering of Temporally Complex Dynamic Scenes https://arxiv.org/abs/2412.06299
% 3. Per-Gaussian Embedding-Based Deformation for Deformable 3D Gaussian Splatting https://arxiv.org/abs/2404.03613
% 4. Grid4D: 4D Decomposed Hash Encoding for High-Fidelity Dynamic Gaussian Splatting https://arxiv.org/abs/2410.20815
% 5. Real-time Photorealistic Dynamic Scene Representation and Rendering with 4D Gaussian Splatting https://arxiv.org/abs/2310.10642
% 6. Spacetime Gaussian Feature Splatting for Real-Time Dynamic View Synthesis https://arxiv.org/abs/2312.16812
% 7. V^3: Viewing Volumetric Videos on Mobiles via Streamable 2D Dynamic Gaussians https://arxiv.org/abs/2409.13648
% 8. Deformable 3D Gaussians for High-Fidelity Monocular Dynamic Scene Reconstruction https://ieeexplore.ieee.org/document/10657752/
% 9. Fully Explicit Dynamic Gaussian Splatting http://arxiv.org/abs/2410.15629
% 11. Gaussian-Flow: 4D Reconstruction with Dynamic 3D Gaussian Particle  https://openaccess.thecvf.com/content/CVPR2024/papers/Lin_Gaussian-Flow_4D_Reconstruction_with_Dynamic_3D_Gaussian_Particle_CVPR_2024_paper.pdf
% 12. A Compact Dynamic 3D Gaussian Representation for Real-Time Dynamic View Synthesis http://arxiv.org/abs/2311.12897

%codebook
% Compact3D: Smaller and Faster Gaussian Splatting with Vector Quantization https://arxiv.org/abs/2311.18159
% Compact 3D Gaussian Representation for Radiance Field https://arxiv.org/abs/2311.13681
% LightGaussian: Unbounded 3D Gaussian Compression with 15x Reduction and 200+ FPS http://arxiv.org/abs/2311.17245
% GaussianImage: 1000 FPS Image Representation and Compression by 2D Gaussian Splatting http://arxiv.org/abs/2403.08551
%End-to-End Rate-Distortion Optimized 3D Gaussian Representation https://arxiv.org/abs/2406.01597

==> ICCV2025-Author-Kit/2_Introduction.tex <==
\section{Introduction}
\vspace{-2mm}
% Dynamic scene rendering is crucial for applications such as virtual reality, augmented reality, gaming, and robotics, where real-time, accurate rendering of moving objects and their environments is vital for creating an immersive experience. Recent advancements in technologies like Neural Radiance Fields~(NeRF)~\cite{mildenhall2021nerf} have enabled high-fidelity scene reconstruction, but at the cost of slow rendering speeds. To address this, 3D Gaussian Splatting (3DGS)\cite{kerbl20233d} significantly enhances rendering speed for each scene, bringing it to real-time levels by representing scenes with 3D Gaussians data.
Dynamic scene rendering is pivotal for applications such as virtual reality, augmented reality, gaming, and robotics, where real-time, precise depiction of moving objects and their environments is essential for an immersive experience. While advancements like Neural Radiance Fields (NeRFs)~\cite{mildenhall2021nerf} have enabled high-fidelity scene reconstruction, they often come with the drawback of slow rendering speeds. To overcome this limitation, 3D Gaussian Splatting (3DGS)~\cite{kerbl20233d} significantly accelerates rendering by representing static scenes with 3D Gaussian data, thereby achieving real-time performance.

% Directly constructing 3D Gaussians per frame incurs prohibitive storage costs~\cite{luiten2024dynamic}. 
% Current some representation methods model the temporal transformation of Gaussians using basis functions (polynomial, Fourier, or learned)~\cite{sun20243dgstream, li2024spacetime, katsumata2024compact}, or extend 3D Gaussians to 4D by incorporating time dimensions~\cite{yang2023real, duan20244d}. These approaches require augmenting each Gaussian with temporally associated attributes, leading to high storage costs. Deformable 3D Gaussian Splatting, on the other hand, decouple dynamic scenes into a canonical 3D Gaussian set and a deformation field \cite{yang2024deformable, huang2024sc, wu20244d, xu2024grid4d, yan20244d}. Representative works, such as 4DGS~\cite{wu20244d}, combine canonical Gaussians and 4D neural voxels Hexplane~\cite{cao2023Hexplane}, achieving competitive reconstruction quality with low storage requirements.


Despite the tremendous success of 3DGS techniques in rendering static scenes, extending them to dynamic scenes using 4D Gaussian Splatting (4DGS) presents significant challenges, with high storage costs emerging as one of the primary concerns~\cite{luiten2024dynamic}. To achieve high fidelity, some approaches either directly model temporal transformations of 3D Gaussian data~\cite{sun20243dgstream, li2024spacetime, katsumata2024compact} or incorporate an additional time dimension~\cite{yang2023real, duan20244d} to generate 4D Gaussian data. However, these methods rely on extensive attributes and impose a substantial storage burden.

To produce a more compact 4DGS format, recent works typically leverage deformable 3DGS techniques to disentangle 4D Gaussian data into a canonical 3D Gaussian set and a Gaussian deformation field~\cite{yang2024deformable, huang2024sc, wu20244d, xu2024grid4d, yan20244d}. In this framework, the deformation field compactly encodes the Gaussian motion and deformation information for each time-step, ensuring that only one canonical 3DGS is maintained. For example, Wu~\etal~\cite{wu20244d} propose a method called 4DGS, which employs compact 4D neural voxels to represent the Gaussian deformation field using variables such as positions, scales and rotations.


% 尽管使用了codebook 但是没有探索codebook内的冗余性，为什么不用anchor那一套
While deformable 3DGS strategies employ compact structures to reduce 4DGS data storage, two major challenges persist. First, redundancy within the structure is not entirely eliminated. For example, even though the deformation field uses compact components such as 4D neural voxels~\cite{cao2023Hexplane}, unexploited spatiotemporal correlations within and across time-steps remain. Second, many practical applications, including mobile VR, require multi-rate compression that allows users to balance rendering quality and file size based on factors such as network bandwidth. This functionality is currently absent in existing deformable 3DGS methods, limiting their broader adoption.
%
To address these concerns, we propose a 4DGS data compression method to further exploits redundancy to push the boundaries of 4DGS compression. We follow the high-level syntax of deformable 3DGS, comprising a canonical 3D Gaussian set and 4D neural voxel components. To exploit redundancy within each component, we incorporate neural contextual coding techniques inspired by the success of neural image compression (NIC) methods~\cite{balle2018variational,balle2016end,minnen2018joint,6,1,12}.

For compressing the 4D neural voxels, which are constructed from multi-resolution grid structures (e.g., Hexplane~\cite{cao2023Hexplane}) with each grid containing a collection of features, we first apply quantization to achieve lossy compression. Next, we disentangle the quantized features into spatial and temporal dimensions. Specifically, the position of each plane $s$ in the coarse-to-fine structure defines the spatial axis, while each plane is partitioned into $t$ rows, with each row representing deformation information of the static scene at a specific time-step, inspired by the 4D neural voxel design~\cite{cao2023Hexplane}.
%
Finally, we introduce a Neural Voxel contextual Coding (NVCC) approach to losslessly compress each individual quantized feature $\bar{\F}_{t}^{s}$, using the compressed features $\hat{\F}_{t}^{s-1}$ from the coarser plane $s-1$ and $\hat{\F}_{t-1}^{s}$ from the previous time-step $t-1$ as spatial and temporal priors, respectively. 
Moreover, to capture long-term temporal dependencies, NVCC maintains a hidden temporal state that updates the temporal prior. By exploiting spatiotemporal correlations, NVCC generates spatiotemporal contexts to produce more accurate estimated distribution $P(\bar{\F}_{t}^{s} | \cdot)$, thereby enhancing contextual coding and lossless compression.
 

% Inspired by video compression methods that compress both motion information and image simultaneously, we approach the compression of 4DGS in two parts: the deformation field and the canonical Gaussian set.

% We begin by examining the deformation field, which uses  Essentially, 4D neural voxels are a collection of features organized in a grid structure, which is crucial and occupies significant storage. Some compression methods reduce redundancy in similar grid structures~\cite{takikawa2022variable,chen2024far} 

% by exploiting spatial correlations within features. To effectively reduce the redundancy of 4D neural voxels, we decompose the 4D neural voxels along both spatial and temporal dimensions. First, we split the voxels into planes of  where coarser planes provide spatial priors for finer ones. Then, we decompose the plane-arranged features along the temporal axis into row-arranged features, allowing previous time points to serve as temporal priors for the current time point. We propose an context model combine both priors to predict the 4D neural voxel distribution, enabling effective entropy encoding.

% Compression has been extensively explored in 3DGS, including techniques such as redundant Gaussian pruning~\cite{lee2024compact, papantonakis2024reducing, navaneet2024compgs, wang2024end}, distillation or compression~\cite{fan2023lightgaussian, wang2024end}, vector quantization~\cite{wang2024end, navaneet2024compgs, lee2024compact, papantonakis2024reducing}, and entropy models ~\cite{chen2024hac, wang2024contextgs}. Many of these methods ~\cite{wang2024end, navaneet2024compgs, chen2024hac, wang2024contextgs} demonstrate their performance in variable bit rate compression. However, this issue remains underexplored in 4DGS. 4DGS~\cite{wu20244d} contains redundancies both in the canonical Gaussian set and the deformation field. 

% The is designed to represent the e, particularly in monocular datasets. For example, in the synthetic dataset, 4DGS~\cite{wu20244d} is initialized with randomly generated points. Methods designed to reduce spatial redundancy in 3DGS may be less effective in this context ~\cite{chen2024hac, lu2024scaffold}. Fortunately, as with traditional Gaussians, the precisions of certain attributes in the canonical Gaussian set affect rendering quality differently, resulting in significant redundancy, with spherical harmonics contributing the most. Although previous work has reduced redundancy through vector quantization~\cite{wang2024end, navaneet2024compgs, lee2024compact, papantonakis2024reducing}, prior methods did not account for the  To further compress the codebook, we propose  which uses a context model for lossless compression by learning latent representations as hyperprior to model the probability of the codebook, thereby enabling entropy encoding

Meanwhile, we compress the canonical 3DGS. While previous studies have explored multi-rate 3DGS data compression~\cite{chen2024hac,wang2024contextgs} by employing neural contextual coding with anchor data structures to cluster 3D Gaussians, these approaches fall short for canonical 3DGS in 4DGS. This is because canonical 3DGS must store information covering entire dynamic scenes for world-to-canonical mapping with the 4D neural voxels~\cite{cao2023Hexplane}, leading to significant sparsity~\cite{wu20244d} that limits the effectiveness of anchor-based methods. Therefore, we adopt a compact 3DGS method that uses vector quantization~\cite{wang2024end, navaneet2024compgs, lee2024compact, papantonakis2024reducing} with an auxiliary quantized codebook to store spherical harmonic information and achieve lossy compression. 
%
However, previous works have overlooked redundancy within the codebook itself. To address this, we introduce a Vector Quantization Contextual Coding (VQCC) methodology that leverages an auxiliary hyperprior feature as context for further losslessly compressing those quantized vectors. To the best of our knowledge, this is the first approach to combine contextual coding with VQ strategies for compressing 3DGS data.

% In the deformation field network, the Hexplane\cite{cao2023Hexplane} module occupies a significant portion of the storage space.Some compression methods target compact grid structures\cite{takikawa2022variable,chen2024far}, which reduce storage redundancy based on the internal similarity of the static scene.However, these methods cannot make good use of the redundancy of the time dimension. It has spatial and temporal relation. Previous work has not considered reducing redundancy through these priors. We propose deformation field context coding(DCC).It introduce an autoregressive context model coupled with both level-wise and neighbor-wise context models.We use these contexts to predict the probability distribution of the Hexplane for facilitating entropy encoding.This method can achieve a highly compact representation of the Hexplane.

By integrating these two novel contextual coding techniques, we introduce the first 4DGS contextual coding framework, 4DGS-CC. Our framework can be optimized for multi-rate compression to meet diverse conditions while significantly reducing storage. Extensive experiments on dynamic scene compression benchmarks, including D-NeRF~\cite{pumarola2021d}, Neu3D~\cite{li2022neural}, and HyperNeRF~\cite{park2021hypernerf}, demonstrate that compared to our baseline 4DGS~\cite{wu20244d}, 4DGS-CC achieves an average storage reduction of approximately $12\times$ while maintaining comparable rendering quality. At the same time, we conducted further experiments with the Saro-GS\cite{yan20244d} method, thereby demonstrating the broader applicability of our approach. Our contributions are summarized as follows:

\begin{itemize}

\item A Gaussian deformation field compression method that disentangles 4D neural voxels into individual features and employs our newly proposed NVCC to exploit spatiotemporal redundancy.

\item A canonical 3DGS compression method, VQCC, which for the first time integrates vector quantization with a contextual coding strategy to reduce redundancy in both the sparse 3DGS data and its associated codebook.

\item A novel 4DGS compression framework, 4DGS-CC, which, to the best of our knowledge, is the first contextual coding method for 4DGS data that achieves multi-rate compression and produces the most compact dynamic scene representation using 4DGS-based methods.

\end{itemize}

==> ICCV2025-Author-Kit/3_Relatedwork.tex <==
\section{Related work}

\begin{figure*}
  \centering
    % \fbox{\rule{0pt}{2in} \rule{1\linewidth}{0pt}}
    \includegraphics[width=1\linewidth]{picture/fig43.pdf}
    \vspace{-2mm}
    \caption{The overview of our 4DGS data compression framework. It consists of six main components, which are decomposition, compression of Canonical Gaussians, compression of 4D neural voxels, lossless decoding, reconstruction and rendering.}
    \vspace{-4mm}
    
  % \hfill
  % \begin{subfigure}{0.28\linewidth}
  %   \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
  %   \caption{Another example of a subfigure.}
  %   \label{fig:short-b}
  % \end{subfigure}
  \label{fig:overview}
\end{figure*}
\noindent\textbf{Dynamic Scene Rendering.} It is a challenging task that creates new views of dynamic scenes from 2D images captured at different times. Recent 3D reconstruction techniques like NeRF and 3DGS have significantly advanced this field. Researchers extended NeRF to 4D for dynamic scene reconstruction~\cite{pumarola2021d, gan2023v4d, park2021hypernerf,fang2022fast}, and later methods decomposed 4D scenes into 2D planes for more compact representations~\cite{wu2024tetrirf, cao2023Hexplane, fridovich2023k}. However, these methods are limited by their rendering efficiency.

To address this issue, 3DGS rendering efficiency is utilized. Extending 3DGS to 4D involves creating 3D Gaussians at each timestamp, but this leads to high storage costs~\cite{luiten2024dynamic}. There are two main methods to extend 3DGS to 4D: explicit and implicit methods. Explicit methods manage the variation of Gaussian properties over time using functions like polynomial, Fourier, or learned functions~\cite{sun20243dgstream, li2024spacetime, katsumata2024compact}, or by adding a time dimension to 3D Gaussian primitives~\cite{yang2023real, duan20244d}. Implicit methods, also called deformable 3DGS~\cite{yang2024deformable, huang2024sc, wu20244d, xu2024grid4d, yan20244d}, separate the scene into a canonical 3D Gaussian set and a deformation field to explain temporal changes. Both methods offer good reconstruction, but explicit methods increase 3DGS primitive attributes, while implicit methods use a compact deformation field for better storage. 4DGS~\cite{wu20244d} is a deformable 3DGS method using a canonical Gaussian set and a deformation field with the Hexplane 4D neural voxels~\cite{cao2023Hexplane}, have demonstrated competitive results with relatively low storage requirements on both multi-view and monocular videos. Despite these improvements, storage of 4DGS data remains a critical bottleneck. To address this, we introduce the 4DGS-CC compression framework, which aims to further reduce storage costs while maintaining high rendering efficiency and reconstruction quality.


\noindent\textbf{Compact radiance field representations.} It have been an important research direction. For NeRF, compact grid~\cite{muller2022instant,cao2023Hexplane,fridovich2023k} structures have been shown to be very effective in reducing network size and improving accuracy, while exploiting contextual dependencies~\cite{chen2024far} between adjacent elements is also a key method for compressing NeRF. Various compression strategies have also been explored for 3D Gaussian fields (3DGS), including redundant Gaussian pruning~\cite{wang2024end,navaneet2024compgs,lee2024compact,papantonakis2024reducing}, spherical harmonic distillation or compression~\cite{fan2023lightgaussian,wang2024end}, vector quantization~\cite{wang2024end,navaneet2024compgs,lee2024compact,papantonakis2024reducing,fan2023lightgaussian}, entropy models, and more. Some approaches have represented Gaussian parameters as 2D grids~\cite{morgenstern2024compact} and applied image compression techniques.

Some works have also focused on developing compact dynamic 3DGS representations. For example, for monocular~\cite{kwak2025modecgsglobaltolocalmotiondecomposition} and multi-view videos~\cite{cho20244dscaffoldgaussiansplatting}, researchers have attempted to achieve compact dynamic 3DGS representations by leveraging the compact structure introduced in~\cite{lu2024scaffold}. However, these approaches do not constitute a multi-rate compression framework. At the same time, although~\cite{kwak2025modecgsglobaltolocalmotiondecomposition} focuses on compact deformable 3D Gaussian representations, it does not attempt to explore the redundancy inherent in 4D neural voxels.
Our method simultaneously accounts for the redundancy present in both the Gaussians and 4D neural voxels, and supports multi-rate compression.


\noindent\textbf{Neural Contextual Coding.}
In modern neural compression frameworks for images and videos, the ability to accurately predict probability distributions through sophisticated entropy modeling is of paramount importance. For instance, a notable study by Minnen et al.~\etal~\cite{minnen2018joint} devised an innovative compression strategy that fuses a hyperprior network with an autoregressive component, thereby capturing intricate spatial correlations within image data to substantially boost compression efficiency. This paradigm, which integrates multiple modeling techniques to better represent data redundancies, has been mirrored in several subsequent compression approaches~\cite{lu2019dvc,hu2021fvc,li2021deep,ChenIntra-Slice,han2024cra5,liu2023icmh,chen2023neural,hu2020improving,Chen_2022_CVPR,liu2025efficient,chen2024group}, further affirming the critical role that neural contextual coding play in advancing the state-of-the-art in data compression research.
Currently, a few works have attempted to apply neural contextual coding for compression in static scene representations, such as those in NeRF~\cite{chen2024far} and 3DGS~\cite{chen2024hac,wang2024contextgs,liu2024hemgs}, achieving promising results. However, these studies have not explored the application of neural contextual coding for compression in dynamic 3DGS scenarios. To the best of our knowledge, we are the first work to apply neural contextual coding techniques to the compression of Gaussian Splatting based dynamic scene representations.
% \noindent\textbf{Compact radiance field representations} has been an important research direction. For NeRF, compact grid structures have been shown to be very effective in reducing network size and improving accuracy, while exploiting contextual dependencies between adjacent elements is also a key method for compressing NeRF. Various compression strategies have also been explored for 3D Gaussian fields (3DGS), including redundant Gaussian pruning, spherical harmonic distillation or compression, vector quantization, entropy models, and more. Some approaches have represented Gaussian parameters as 2D grids and applied image compression techniques.

% However, the parameters of 4DGS consist of a typical Gaussian set and a deformation field network, which differs from both static 3DGS and NeRF, so existing methods may not be suitable for 4DGS. This paper aims to develop a compression method for both the Gaussian set and the deformation field network. To the best of our knowledge, our method is the first in the field of 4DGS compression and represents the current smallest storage 4DGS.


==> ICCV2025-Author-Kit/4_1Methodology.tex <==
\section{Methodology}




==> ICCV2025-Author-Kit/4_2Methodology.tex <==
\vspace{-2mm}
\subsection{Preliminaries}
\vspace{-2mm}

  % \begin{subfigure}{0.48\linewidth}
  %   \includegraphics[width=1\linewidth]{ICCV2025-Author-Kit/picture/fig19.pdf}
  %   \caption{Overview of our context model for Hexplane.Plane interpolated feature at the corresponding position in the previous layer to obtain the level context.We keep a latent $H_t$,Each time a feature at a specific timestep $L_t$is decoded, it is used to update the latent representation to get $H_{t+1}$, which then serves as the neighbour context for decoding the feature at the next timestep $L_{t+1}$.}
  %   \label{fig:dcc}
  % \end{subfigure}

In this study, we follow the deformable 3DGS methodology~\cite{wu20244d, yan20244d} to decompose 4DGS data into \textit{canonical 3DGS data} and a \textit{Gaussian deformation field}, which are subsequently compressed using \textit{Neural contextual Coding} techniques. In this section, we briefly review these three methodologies.

\noindent\textbf{Canonical 3DGS data.} 
In the deformable 3DGS framework, the canonical 3DGS data represents a sparse variant of the 3DGS data that encapsulates information covering the entire dynamic scene. Specifically,
3DGS is a technique for representing 3D scenes as point cloud, where each point is associated with a full 3D covariance matrix, $\Sigma$ centered at $\mathcal{X}$ to represent a Gaussian function $G(\mathcal{X})=e^{-\frac{1}{2} \mathcal{X}^T \Sigma^{-1} \mathcal{X}}$. 
%
To facilitate differentiable optimization, the covariance matrix $\Sigma$ is factorized as $\Sigma = R^T S^T S R$, where $S$ and $R$ are scaling and rotation matrix parameterized by the vector $s$ and $r$, respectively. 
%
Each Gaussian is assigned an opacity $\alpha$ and a view-dependent color, represented using spherical harmonics $\mathcal{C}$, which are used to compute the pixel values during rendering.
Hence, we will only use the location $\mathcal{X}$ and attributes $s$, $r$, $\alpha$, $\mathcal{C}$ to characterize the 3DGS data.


% Finally, the 3D Gaussians are splatted onto the 2D plane, and the pixel values are computed based on $\alpha$ and $\mathcal{C}$.
% %
% In summary, each 3DGS data can be characterized by the following attributes
%
% During rendering, each 3D Gaussian is first projected onto a 2D space using a view transformation. An affine approximation is obtained via its Jacobian, from which the projected centers and 2D covariances are computed. These primitives are then depth-sorted. 








% Here, $c_i$, $\alpha_i$ represents the density and color of this point computed by Gaussian $G$ multiplied by an optimizable per-point opacity $\alpha$ and 
% where \( c_i \) is the color of the \( i \) -th Gaussian, calculated from spherical harmonic coefficients $C$. The opacity \( \alpha_i \) is obtained by the 2D Gaussian distribution function at the position of the pixel multiplied by its optimizable opacity $\alpha$.
\label{Vector quantization Contextual coding}
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{picture/fig41.pdf}
\vspace{-3mm}
   \caption{Overview of Vector Quantization Contextual Coding.}
\vspace{-3mm}
    \label{fig:VCC}
\end{figure}
\label{Gaussian Deformation Field}
\noindent\textbf{Gaussian Deformation Field}. In our work, we primarily follow the framework presented in~\cite{wu20244d,yan20244d}, which employs 4D neural voxels to store spatiotemporal information for robust rendering in both monocular and multi-view scenarios.
Specifically, we employ the 4D neural voxels method described in~\cite{cao2023Hexplane}. For a given time-step \(t\), we concatenate \(t\) with the spatial coordinates $\mathcal{X}$ of each Gaussian and query the 4D neural voxels to retrieve the corresponding feature. This feature is then processed by the MLPs to generate the deformation parameters
$\{\Delta\mathcal{X}, \Delta{s}, \Delta{r}, \Delta\alpha, \Delta\mathcal{C}\}$ by using MLPs. 
The resulting deformation information is subsequently fused with the \textit{canonical 3DGS data} to produce deformed Gaussians, which are used to render the novel-view image at time-step $t$.


% Specifically, it includes planes $P^l=\left\{P_{x, y}^l, P_{y, z}^l, P_{x, z}^l,P_{x, t}^l, P_{y, t}^l, P_{z, t}^l\right\}$, where \( P_{i,j}^l \in \mathbb{R}^{h \times l N_i \times l N_j} \). Here, \( h \) represents the hidden dimension of the features, \( N \) denotes the base resolution of the voxel grid, and \( l \) equals the upsampling ratio. By default, \( l \in \{1, 2\} \), but it may vary in different scenes.

% For a 4D sample point $p=(x,y,z,t)$, we performs interpolation based on its projected coordinates on six planes to obtain the corresponding features $f(p)$ of the point as \cite{wu20244d}.
% \begin{equation}
% \begin{aligned}
% f(p) &= \bigcup_l\prod_{i, j} \psi_{b i}\left(\pi_{i, j}(p) ; P_{i, j}^l\right) \\
% (i, j) & \in \{(x, y), (x, z), (y, z), (x, t), (y, t), (z, t)\}
% \end{aligned}
% \end{equation}
% $\psi_{b i}$ represents bilinear interpolation, and $\pi_{i, j}(p)$ denotes the projected coordinates of sample point $p$ on $P_{i, j}^l$ .


% After obtaining the encoded features $f(p)$ of the 3D Gaussian, a multi-head Gaussian deformation decoder $\mathcal{D} = \left\{\phi_x, \phi_r, \phi_s, \phi_o, \phi_c\right\}$ is employed to compute required variables. The variations in several attributes are calculated using MLPs, $\Delta V = \phi_V\left(f(q)\right)$. The deformed Gaussian's $V$ attribute can be represented as: $V^\prime = V + \Delta V$. Here, $V$ denotes the attributes of the Gaussian $V \in \{\mathcal{X}, \mathcal{C}, \alpha, r, s\}$. Among them, $C$ and $\alpha$ are optional.


\label{Neural Contextual Coding}
\noindent\textbf{Neural Contextual Coding.}
We employ neural contextual coding techniques to losslessly compress a given quantized content $\bar{\A}$. According to information theory~\cite{shannon1948mathematical}, the cross entropy $H(q,p) = \mathbb{E}_{\bar{\A} \sim q} \left[-\log(p(\bar{\A}))\right] $ serves as a practical lower bound on the storage cost for losslessly compressing $\bar{\A}$. Here, $p(\bar{\A})$ denotes the estimated probability distribution of  $\bar{\A}$, while $q(\bar{\A})$, represents its true distribution. By refining $p(\bar{\A})$  to more closely approximate $q(\bar{\A})$, we can reduce $H(q,p)$, and consequently lower the storage cost. This procedure is known as entropy coding, where, in our work, the conditional probability $p(\bar{\A} | \cdot)$  is modeled based on previously compressed contents.
%

\vspace{-1mm}


\subsection{Overview}
\vspace{-1mm}
Here, we employ the deformable 3DGS framework as in 4DGS~\cite{wu20244d} to demonstrate our 4DGS-CC framework, as illustrated in Fig.~\ref{fig:overview}. It is worth noting that our methodology should be theoretically applicable to other deformable 3DGS frameworks. For instance, in our implementation, we also build upon the latest method SaRO-GS~\cite{yan20244d}.

\textbf{Decomposition.} We first decompose the dynamic scene into two primary components: Canonical Gaussians and a Gaussians deformation field (\ie, 4D neural voxels), each of which will be compressed separately.

%
\begin{figure}[t]
  \centering
   \includegraphics[width=1\linewidth]{picture/fig42.pdf}
\vspace{-3mm}
   \caption{Overview of Neural Voxels Contextual Coding.}
\vspace{-3mm}

    \label{fig:VCC}
\end{figure}
\textbf{Canonical Gaussian Compression.} The Canonical Gaussian data is characterized by the location $\mathcal{X}$ and attributes including scaling $s$, rotation $r$, and opacity $\alpha$, which will be compressed using a hybrid lossy–lossless compression scheme.
Specifically, $\mathcal{X}$ is first quantized at 16 bits and  $s, r$ and $\alpha$ quantized to 8 bits to achieve lossy compression, which will be losslessly stored directly.

For the lossy compression of the spherical harmonics $\mathcal{C}$,
we adopt a vector quantization strategy as described in~\cite{navaneet2024compgs}, which encodes the information into indices and a codebook. The indices are further losslessly compressed using a run-length coding algorithm into the bit-stream. Meanwhile, the codebook $\cY$ is first quantized into $\bar{\cY}$ , then is losslessly compressed using our VQCC strategy, which leverages a learned hyper-prior for lossless contextual coding. Detailed information about the VQCC is provided in \textit{Section~\ref{Vector quantization Contextual coding}}.



\textbf{4D Neural Voxel Compression.}
The 4D Neural Voxels are constructed as a set of multi-resolution Hexplanes. Their compression also follows a hybrid lossy–lossless scheme similar to the compression of Canonical Gaussian. Initially, we apply the quantization strategy proposed in~\cite{balle2018variational} directly to the 4D Neural Voxels for the lossy compression. Next, the quantized 4D Neural Voxels are decomposed into individual quantized latent features $\bar{\f}_t^s$, where the spatial dimension $s$ corresponds to the $s$-th level in a coarse-to-fine hierarchy, and the temporal dimension $t$ corresponds to the $t$-th row in each Hexplane storing the deformation information for a specific static scene at a given time-step inspired by~\cite{cao2023Hexplane}. 
%
To losslessly compress each individual quantized feature $\bar{\f}_t^s$, we introduce an innovative NVCC approach that leverages spatial and temporal priors, the compressed feature $\hat{\f}_{t}^{s-1}$ from the coarser plane $s-1$ and the compressed feature $\hat{\f}_{t-1}^{s}$ from the previous time-step $t-1$ as spatial and temporal priors, respectively. Detailed information on the NVCC approach is provided in \textit{Section~\ref{NVCC}}.

%
\textbf{Lossless Decoding}. 
During the decompression stage, all bit-streams are losslessly decoded. Here, we can obtain the decoded location $\mathcal{\hat{X}}$ and the decoded attributes $\hat{s}, \hat{r}, \hat{\alpha}$. To losslessly decode the codebook and feature  $\hat{\f}_t^s$, we employ an entropy decoding algorithm that reconstructs the vectors from the bit-stream using the estimated distributions produced by VQCC and NVCC, respectively. Detailed information is provided in the supplementary materials.

\textbf{Reconstruction.}
With compressed indices and codebook, we can assemble the reconstructed spherical harmonics $\mathcal{\hat{C}}$, which will be combined with compressed location $\mathcal{\hat{X}}$ and compressed attributes $\hat{s}, \hat{r}, \hat{\alpha}$ to obtain the reconstructed Canonical 3DGS data using the operations in~\cite{navaneet2024compgs}. Meanwhile, with those compressed features $\bar{\f}$, we can re-assemble the reconstructed 4D Neural Voxels. 

\textbf{Rendering.}
We use both reconstructed 4D Neural Voxels and Canonical 3DGS data to render the novel-view image at time-step $t$ using the standard operations as in \textit{Section~\ref{Gaussian Deformation Field}}.  




% \begin{figure}[t]
%   \centering
%   % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    \includegraphics[width=1\linewidth]{picture/fig2.pdf}

%    \caption{The details of Vector quantization Contextual coding. We adopted the vector quantization method, obtained codebook and encoding indices of the Gaussians.We randomly initialize latents $z$ for codebook $y$.Then quantized them.Using the context $\hat{z}$, we model the probability of the quantized $\hat{y}$ for entropy coding.$\hat{z}$ itself is also encoded by entropy coding.}
%    \label{fig:VCC}
% \end{figure}

% \begin{figure*}
%   \centering
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=1\linewidth]{picture/fig5.pdf}
%     \caption{Overview of our context model for Hexplane.The left side of the figure shows the context model for spatio-only planes while the right side shows that for spatiotemporal planes.Both planes interpolated feature at the corresponding position in the previous layer to obtain the level context.For spatio-only planes we select the previous row’s three nearest features as neighbour context.For spatiotemporal planes,we keep a latent $H_t$,Each time a feature at a specific timestep $L_t$is decoded, it is used to update the latent representation to get $H_{t+1}$, which then serves as the context for decoding the feature at the next timestep $L_{t+1}$.The box on the right shows our specific update process.}
%     \label{fig:dcc}
%   % \hfill
%   % \begin{subfigure}{0.2\linewidth}
%   %   % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%   %   \caption{Another example of a subfigure.}
%   %   \label{fig:short-b}
%   % \end{subfigure}
%   % \caption{Example of a short caption, which should be centered.}
%   % \label{fig:short}
% \end{figure*}



% Canonical Gaussian set compression. We first applied Quantization-aware training to optimize the model by simulating the quantization process, ensuring that it maintains accuracy as much as possible during final quantization. We used 16-bit float precision for positional attributes and b-bit asymmetric quantization for geometric attributes. For spherical harmonic, we employed k-means-based vector quantization. To further eliminate redundancy in the spherical harmonic after vector quantization, we introduced a context model to probabilistically model the codebook, and finally used an entropy model for encoding. The indices are encoded using run-length encoding.

% Deformation field network compression.We focused primarily on reducing the redundancy in the hexplane. To facilitate the quantization required for entropy encoding, we also used Quantization-aware training. Afterward, we leveraged the inter-plane and intra-plane correlations of the hexplane to design a context model. Through the context model and a learnable neural network, we performed autoregressive probabilistic modeling of the hexplane, and finally applied entropy encoding for both encoding and decoding.


% Deformation field Contextual coding. On deformation field network compression, we focused primarily on reducing the redundancy in the 4D neural voxels. To facilitate the quantization required for entropy encoding, we also used quantization-aware training. Afterward, we decompose the grid into rows along the temporal axis ,so we can leverage row-wise context dependencies.Additionally, we incorporate context dependencies across different resolution levels.We propose an autoregressive context model combine these contexts dependencies to predict the 4D neural voxels distribution row by row, enabling effective entropy encoding.

% Quantization-aware training and opacity regulation for canonical Gaussian. We first applied Quantization-aware training to optimize the model by simulating the quantization process, ensuring that it maintains accuracy as much as possible during final quantization. We used 16-bit float precision for positional attributes and b-bit asymmetric quantization for geometric attributes.Follow previous job\cite{navaneet2024compgs,zhang2024mega} we add a regularization term based on the opacity values,$L_{opa} = \sum_{i} \sigma_i$,to encourage opacity values close to zero. During optimization, we prune Gaussians that exhibit near-zero opacity.


% Vector quantization Contextual coding.For the spherical harmonic of the canonical Gaussian, we employed vector quantization based on the k-means algorithm, obtaining the corresponding codebook and indices for the spherical harmonic.To further reduce redundancy in the spherical harmonic after vector quantization, we introduced a context model to predict the probability distribution of codebook, followed by the use of arithmetic encoding for compression. The indices are encoded using run-length encoding.

% Quantization-aware training.

% Gaussian Pruning.

% Vector Quantization.

% Build context model.

% Entropy coding.

% Gaussian is defined by 59 parameters. The mean $\mathcal{X} \in \mathbb{R}^{3}$ captures the rough outline of the scene, while the opacity $\alpha$, rotation $r$ and scaling $s$ govern the rendering process during rasterization. These quantities are unified in $F \in \mathbb{R}^{8}$. Together, $\mathcal{X}$ and $F$ describe geometry of the scene , and the spherical harmonic (SH) coefficients $\mathcal{C}$ assign view-dependent colors. In terms of sensitivity, position $\mathcal{X}$ is the most critical, followed by geometry $F$, with color $\mathcal{C}$ being the least sensitive.


% In 4DGS, each Gaussian is defined by 59 parameters. The mean $\mathcal{X} \in \mathbb{R}^{3}$ captures the rough outline of the scene, while the opacity $\alpha$, rotation $r$ and scaling $s$ govern the rendering process during rasterization. These quantities are unified in $F \in \mathbb{R}^{8}$. Together, $\mathcal{X}$ and $F$ describe geometry of the scene , and the spherical harmonic (SH) coefficients $\mathcal{C}$ assign view-dependent colors. In terms of sensitivity, position $\mathcal{X}$ is the most critical, followed by geometry $F$, with color $\mathcal{C}$ being the least sensitive.

% For the position information $\mathcal{X}$, we use 16-bit float precision to maintain reconstruction fidelity. For the geometric information $F$, we employ b-bit asymmetric quantization, where the scaling factor $\gamma_i$ and the offset factor $\beta_i$ are learned during fine-tuning:
% \begin{equation}
% \begin{split}
% \hat{F}_i^n &= \left\lfloor \operatorname{clamp}\left(\frac{F_i^n - \beta_i}{\gamma_i}, 0, 2^b - 1\right) \right\rceil \\
% \bar{F}_i^n &= \hat{F}_i^n \times \gamma_i + \beta_i
% \end{split}
% \end{equation}

% where $i \in \{0, 1, 2, \dots, 7\}$.After training, $F$ will be encoded with b-bit quantization, while $\gamma_i$ and $\beta_i$ will be stored in full precision.


==> ICCV2025-Author-Kit/4_3Methodology.tex <==
\subsection{Vector quantization Contextual Coding}
\vspace{-1mm}

To losslessly compress the quantized codebook $\bar{\cY} = \{\bar{\y}_i\}$ we adopt a VQCC strategy as illustrated in Fig.~\ref{fig:VCC}. Inspired by the hyper-prior contextual coding techniques in neural image compression~\cite{balle2018variational}, we learn a hyper-prior feature $\z_i$ for each quantized code $\bar{\y}_i$. 
This hyper-prior feature is then quantized to produce $\bar{\z}_i$ and losslessly compressed using the uniform entropy coding algorithm as in~\cite{balle2016end} and subsequently losslessly compressed using the uniform entropy coding algorithm described in~\cite{balle2016end}, resulting in a compressed hyper-prior feature $\hat{\z}_i$. 
%
The compressed hyper-prior is used as prior information to estimate the distribution $p(\bar{\y}_i| \hat{\z}_i)$, where the distribution is parameterized by learned mean and variance vectors produced by MLPs, as detailed in~\cite{balle2018variational}. With the estimated distribution $p(\bar{\y}_i| \hat{\z}_i)$, we perform an entropy coding procedure outlined as in~\textit{Section~\ref{Neural Contextual Coding} on Neural Contextual Coding}, to losslessly transmit $\bar{y}_i$ into a bit-stream. To the best of our knowledge, this is the first work to investigate redundancy within the codebook by incorporating a hyper-prior in the 3DGS data compression research.

% We adopted the vector quantization method using the K-means algorithm, following\cite{navaneet2024compgs}. During training, we store unquantized parameters $\mathcal{C}$ and quantize them in the forward pass, using the quantized parameters $\hat{\mathcal{C}}$ for rendering and loss computation. In the backward pass, we apply the straight-through estimator (STE) to propagate gradients to the unquantized parameters. After training, only the codebook and encoding indices of the Gaussians are retained. The K-means algorithm alternates between updating codebook and indices, with codebook updated after each iteration and indices updated every $100$ iterations for faster training.

% To further compress the spherical harmonic, we use a context model to apply additional lossless compression. For the codebook $y \in \mathbb{R}^{N \times 48}$, we sample random learnable vectors from the standard normal distribution as its hyperprior $z \in \mathbb{R}^{N \times k}$, where $k < 48$ represents the latent dimension. In practice, $k=6$. We quantized $y,z$ with $q_y,q_z$ to $\hat{y},\hat{z}$
% Using the hyperprior $\hat{z}$, we model the probability of the quantized $\hat{y}$ for entropy coding. We model $P(\hat{y}_i | \hat{z}_i)$ as a Gaussian distribution with mean $\mu_i$ and standard deviation $\sigma_i$, and use a tiny MLP to predict $\mu_i \in \mathbb{R}^{48}, \sigma_i \in \mathbb{R}^{48}$ from $\hat{z}_i$.
% Simultaneously, we assume that $z \sim \mathcal{N}(0, I)$.Therefore, we can calculate $p\left(\hat{y}_i\right)$,$p\left(\hat{z}_i\right)$ as equation \ref{eq:probability}. Therefore, the entropy loss is calculated as:
% \begin{equation}
%     L_{\text{code}} = \sum_{i=1}^N \left[\left(- \log_2 p\left(\hat{y}_i\right)\right)+\left(- \log_2 p\left(\hat{z}_i\right)\right)\right]
% \end{equation}
% We only train the entropy model after the training is completed, so it does not consume too much time.
% \begin{equation}
% \begin{aligned}
% p\left(\hat{y}_i\right) &= \int_{\hat{y}_i - \frac{1}{2} q_y}^{\hat{y}_i + \frac{1}{2} q_y} \phi_{\mu_i, \sigma_i}(x) \, dx \\
% &= \Phi_{\mu_i, \sigma_i}\left(\hat{y}_i + \frac{1}{2} q_y\right) - \Phi_{\mu_i, \sigma_i}\left(\hat{y}_i - \frac{1}{2} q_y\right) \\
% & \mu_i, \sigma_i = \text{MLP}(\hat{z}_i)
% \end{aligned}
% \end{equation}
% Here, $\phi$ represents the probability density function and $\Phi$ is the cumulative distribution function. Therefore, we define the entropy loss as the bit cost for $\hat{y}$:
% \begin{equation}
% L_{\text{code-entropy}} = \sum_{i=1}^N \left(- \log_2 p\left(\hat{y}_i\right)\right)
% \end{equation}


% Since 3DGS models the scene as a set of Gaussians, the ordering of these Gaussians is not important. Therefore, we sort the Gaussians by indices, so that Gaussians with the same code appear together in the list. Then, we use run-length encoding, which compresses by replacing consecutive identical values with a combination of the value and its frequency of occurrence. Since we only have one set of indices, the final storage of the indices becomes very small and can be almost ignored.

==> ICCV2025-Author-Kit/4_4Methodology.tex <==
\subsection{Neural Voxels Contextual Coding}
\label{NVCC}
\vspace{-1mm}

% Our goal is to minimize the entropy of the 4D neural voxels to reduce bits needed for encoding, such as with arithmetic coding.We take into account that at different resolution levels, features from high-resolution planes are correlated with the features at the corresponding positions in low-resolution planes. Furthermore, within a single plane, there is strong temporal correlation between features in adjacent rows.This motivates us to use a context model in encoding the 4D neural voxels module.

%loss


%%

% Our method consists of three main parts: the quantization module, the level context model, and the neighbor context model.

To losslessly compress each quantized feature $\bar{\f}_t^s$ at $s$-th plane and $t$-th time-step (\ie, row), we introduce the NVCC methodology, which exploits the spatiotemporal redundancy inherent in the neural voxel. 
%
Similar to VQCC, we adopt a hyperprior contextual coding paradigm, where  $\bar{\f}_t^s$ is iteratively entropy coded using NVCC. Specifically, when compressing $\bar{\f}_t^s$, we utilize the compressed feature $\hat{\f}_{t}^{s-1}$ from the coarser plane $s-1$ as the spatial prior and the compressed feature $\hat{\f}_{t-1}^{s}$ from the previous time step $t-1$ as the temporal prior.
% \begin{figure}[t]
%   \centering
%    \includegraphics[width=1\linewidth]{ICCV2025-Author-Kit/picture/fig42.pdf}

%    \caption{Overview of Neural Voxels Contextual Coding.}
%     \label{fig:VCC}
% \end{figure}
Using only the temporal prior $\hat{\f}_{t-1}^{s}$ at $t-1$ without proper alignment can introduce temporal disparity. To improve temporal consistency, we leverage long-term dependencies by incorporating more additional temporal priors, denoted as $\{\hat{\f}_{i}^{s}|i<t\}$. However, conditioning on all previously compressed temporal priors $\{\hat{\f}_{k}^{i}| i<t\}$ becomes impractical when dealing with a large number of time-step $t$. Inspired by~\cite{ChenIntra-Slice}, we adopt a recurrent architecture and introduce latent features $\h_t^s$ to summarize the accumulated information before time-step $t$. During our implementation, when coding $\bar{\f}_{t}^{s}$, we employ the following cross-attention mechanism to align the temporal prior  $\hat{\f}_{t-1}^{s}$ with the hidden feature $\h_{t-1}^s$ yielding a new hidden feature $\h_{t}^s$. This updated hidden feature will serve as an enhanced temporal prior for coding $\bar{\f}_t^s$ and will be iteratively fused with the compressed feature $\hat{\f}_{t}^{s}$ during the coding of $\bar{\f}_{t+1}^{s}$ at $t+1$. The final estimated distribution is defined as $p(\bar{\f}_t^s | \h_t^s, \hat{\f}_t^{s-1})$.

\vspace{-2mm}
\begin{equation}
\begin{split}
&\mathbf{q_t} = W_q \cdot \mathbf{h}_{t-1}^s,
\mathbf{k_t} = W_k \cdot \hat{\mathbf{f}}_{t-1}^{s},
\mathbf{v_t} = W_v \cdot \hat{\mathbf{f}}_{t-1}^{s},\\
&\mathbf{h}_{t}^s = \text{Softmax}\left(\frac{\mathbf{q_t} \cdot \mathbf{k_t}^T}{\sqrt{d}}\right) \cdot \mathbf{v_t} + \hat{\mathbf{f}}_{t-1}^{s}, 
\end{split}
\end{equation}
where $W_q,W_k,W_v$ are learnable projection matrices and $d$ represent the dimension of the vector $\mathbf{q}_t$.


Note that the first quantized feature $\bar{\f}_1^1$ at the first plane and the first time step is entropy coded using a uniform distribution $p(\bar{\f}_1^1)$ as in~\cite{balle2016end}. For the remaining features at the first plane, only temporal priors are available, and their estimated distribution is given by $p(\bar{\f}_t^1 | \h_{t}^1)$. In contrast, features at the first time step are encoded solely using spatial priors, yielding an estimated distribution $p(\bar{\f}_1^s|\hat{\f}_{t}^{s-1})$. Moreover, since we adopt the deformable 3DGS framework from~\cite{wu20244d,yan20244d}, which comprises six neural voxels and three of which are purely spatial by design, therefore the estimated distributions for these spatial-only voxels are produced exclusively using spatial priors.

% Inspired by \cite{chen2024far}, the lower-resolution planes can helps us to predict fine features in higher-resolution planes. Specifically, for the grid vertex $n_{v_1,v_2}$ at position $v_1,v_2$ in $P_{i,j}^l$, its context depends on the interpolated feature $f$ at the corresponding position $q_{v_1,v_2}$ in the previous layer. For the first layer of the plane, we set its context to be all-ones vectors to align with the input of network.

% We aim to capture the temporal redundancy within planes in more detail by expanding the receptive field of its neighbor context. Let $P_{i,j}^l \in \mathbb{R}^{h \times l N_T \times l N_S}, (i,j) \in \{(x,t), (y,t), (z,t)\}$, where $N_T, N_S$ represent the temporal and spatial dimensions of the spatiotemporal planes. We treat all vertexes at a given time as a whole, $P_{i,j}^l = \{L_1, L_2, ..., L_{lN_T}\}$, where $L_t \in \mathbb{R}^{h \times l N_S}$. In theory, all previous features can help model the conditional distribution of the current feature $L_t$, i.e., $p(L_t | L_{<t})$. However, using a probability model that includes all previously encoded features is clearly impractical.Inspired by \cite{ChenIntra-Slice}, we introduce a set of latent features $\{H_t\}_{t=1:lN_T}$ to summarize features of all previous time, and we model the conditional probability of $L_t$ as $p(L_t | H_t)$. This allows us to establish an entropy model $p(P_{i,j}^l)$ using a recurrent framework.
% % $\{L_1, L_2, ..., L_{t-1}\}$ %
% We use an attention-based gated network to integrate $H_t$ and $L_t$.
% This allows us to update the latent using the feature of current time. Finally, we add the result to the weighted feature tensor $L_t$ for the current time, obtaining $H_{t+1}$. For \( H_{1} \), we initialize it as a vector of ones.


% In summary, in the spatiotemporal plane, the position of the grid vertex $n_{v_1,v_2}$ at $(v_1, v_2)$ has its context as $n_{tem} = H_{v_1,v_2}$.

% By combining the level context and the neighbor context, we can concatenate them to obtain the final context, $c_{v_1,v_2} = \operatorname{concat}(f, n)$. For the spatial-only plane, $n$ is $n_{spa}$, and for the spatiotemporal plane, $n$ is $n_{tem}$. We then use a tiny MLP to predict $\mu_{v_1,v_2}, \sigma_{v_1,v_2}$ from $c$, allowing us to compute $p\left(n_{v_1,v_2}\right)$ as equation \ref{eq:probability}.
% % \begin{equation}
% % \begin{aligned}
% % p\left(n_{v_1,v_2}\right)  =& \int_{n_{v_1,v_2}-\frac{1}{2} q}^{n_{v_1,v_2} + \frac{1}{2} q} \phi_{\mu_{v_1,v_2}, \sigma_{v_1,v_2}}(x) dx \\
% %  =& \Phi_{\mu_{v_1,v_2}, \sigma_{v_1,v_2}}\left(n_{v_1,v_2} + \frac{1}{2} q\right) -\\& \Phi_{\mu_{v_1,v_2}, \sigma_{v_1,v_2}}\left(n_{v_1,v_2} - \frac{1}{2} q\right) \\
% % & \mu_{v_1,v_2}, \sigma_{v_1,v_2} = \text{MLP}(c_{v_1,v_2})
% % \end{aligned}
% % \end{equation} 
% % Here, $\phi$ represents the probability density function, and $\Phi$ represents the cumulative probability function. 
% Therefore, we can define its entropy loss, and the bit cost of $\hat{y}$ is:
% \begin{equation}
% L_{\text{Hexplane}} = \sum \left( - \log_2 p\left(n_{v_1,v_2}\right) \right)
% \end{equation}

==> ICCV2025-Author-Kit/4_5Methodology.tex <==
%%loss
\vspace{-1mm}
\subsection{Optimization}
\vspace{-1mm}
We optimize our 4DGS-CC framework by jointly minimizing both the original loss from the 4DGS baseline models and an additional storage-related loss, as detailed below.
\begin{equation}
\mathcal{L} = \mathcal{L}_{\mathrm{4DGS}} + \lambda_e \mathcal{L}_{\mathrm{voxels}} + \lambda_c \mathcal{L}_{\mathrm{code}}.
\end{equation}

Here, \(\mathcal{L}_{\mathrm{4DGS}}\) denotes the original 4DGS loss~\cite{wu20244d,yan20244d}, which primarily comprises a rendering optimization term that quantifies the discrepancy between the rendered and ground-truth images, along with several regularization terms to enhance the quality. Additionally, $\mathcal{L}_{\mathrm{code}}$ and $\mathcal{L}_{\mathrm{voxels}}$ represent the storage costs for the compressed codebook and neural voxels, respectively. We optimize these costs by directly minimizing the cross-entropy values produced by the VQCC and NVCC modules, thereby enabling differentiable optimization following NIC methods~\cite{balle2018variational,balle2016end,minnen2018joint,1,6}. The user-specific hyperparameters $\lambda_e$ and $\lambda_c$ balance these components to achieve an optimal storage-distortion trade-off under varying storage requirements.
% \begin{equation}
% L_{\text{code}} = \sum_{i=1}^N \left[\left(- \log_2 p(\bar{\y}_i| \bar{\z}_i)\right)+\left(- \log_2 p\left(\bar{\z}_i\right)\right)\right]
% \end{equation}
% \begin{equation}
% L_{\text{voxel}} = \sum \left( - \log_2 p\left(\right) \right)
% \end{equation}


% Here, $L_{\mathrm{4DGS}}$ represents the rendering loss defined in 4DGS\cite{wu20244d}, which includes fidelity penalty loss terms and a grid-based total variation loss. The second part of equation estimated bits for the anchor attributes $L_{\mathrm{entropy}}$. The final term $L_{opa}$ controls the sparsity of the opacity. $\lambda_e$ and $\lambda_{opa}$ are hyperparameters used to balance the loss components. We incorporate different techniques or loss terms at various iteration steps to stabilize the training process.$L_{\mathrm{code}}$ is only used after Gaussian parameters and the deformation field optimization.

% In the encoding/decoding process, for canonical Gaussian set position and geometric information, we directly save the quantized results. For color information, we first encode/decode its latent variable $\hat{z}$ using arithmetic coding, and then use a context model to predict the Gaussian distribution the codebook $\hat{y}$ to derive the used for arithmetic coding. In hexplane compression, we encode and decode each plane row by row in the order from the lowest to the highest resolution. The decoding result of the previous row provides the context for the decoding of the next row, which is an autoregressive process.

==> ICCV2025-Author-Kit/5_experiment.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}

\vspace{-2mm}
\begin{tabular}{lcccc}
\noalign{\hrule height 1pt}
\rowcolor[HTML]{FFFFFF} 
\textbf{Methods} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{Size$\downarrow$} \\
\noalign{\hrule height 1pt}
TiNeuVox-B~\cite{fang2022fast}       & 32.67 & 0.97  & 0.040      & 48    \\
Hexplane~\cite{cao2023Hexplane}        & 31.04 & 0.97  & 0.040      & 38    \\
V4D~\cite{gan2023v4d}              & 33.72 & 0.98  & 0.020      & 377   \\
Kplanes~\cite{fridovich2023k}          & 31.61 & 0.97  & -         & 418   \\ \hline
4DGS~\cite{wu20244d}             & 34.07 &   \cellcolor{pink}{0.979} & 0.026     & 23.3 \\
Saro-GS~\cite{yan20244d}          & \cellcolor{pink}{35.04} & 0.977 & \cellcolor{pink}{0.025}     & 49.9 \\
C-D3DGS~\cite{katsumata2024compact}          & 32.19 & -     & 0.040      & 159 \\
Real-time 4DGS~\cite{yang2023real}   & 31.32 & 0.961 & 0.043     & 1068
\\ \hline
Ours (4DGS) high    & 34.12 & \cellcolor{yellow}{0.978} & 0.028     & 1.9   \\
Ours (4DGS) mid     & 33.99 & 0.977 & 0.029     & \cellcolor{yellow}{1.8}   \\
Ours (4DGS) low     & 33.94 & 0.977 & 0.030      & \cellcolor{pink}{1.7}   \\
Ours (Saro-GS) high & \cellcolor{yellow}{34.9}  & 0.976 & \cellcolor{yellow}{0.026}     & 5.6   \\
Ours (Saro-GS) mid  & 34.79  & 0.976 & 0.027     & 4.9 \\
Ours (Saro-GS) low  & 34.69 & 0.976 & 0.028     & 4.4  \\
\noalign{\hrule height 1pt}
\end{tabular}
\vspace{-1mm}
\caption{Quantitative comparison results on D-NeRF dataset. The best and second-best results are highlighted in \colorbox{pink}{\textcolor{black}{red}} and \colorbox{yellow!50}{\textcolor{black}{yellow}} cells, respectively. Size values are measured in megabytes (MB). At three distinct storage levels, our 4DGS variant achieves compression ratios of $\textbf{12.3}\times$, $\textbf{12.9}\times$, and $\textbf{13.7}\times$ , while our Saro-GS variant achieves compression ratios of $\textbf{8.9}\times$,$\textbf{10.2}\times$,$\textbf{11.3}\times$, compared to baseline methods 4DGS and Saro-GS.}
\label{d-nerf}
\vspace{-2mm}

\end{table}

\vspace{-1mm}
\section{Experiment}
\vspace{-1mm}

% \subsection{Datasets}
% We conducted comprehensive experiments on two monocular datasets, D-NeRF~\cite{pumarola2021d} and HyperNeRF datasets~\cite{park2021hypernerf}, and one multi-view dataset, Neu3D~\cite{li2022neural}. The monocular video dataset D-NeRF~\cite{pumarola2021d} is a synthetic dataset specifically designed for monocular settings, where camera poses are generated in a near-random manner for each timestamp, while the HyperNeRF dataset~\cite{park2021hypernerf} uses points computed by SfM from 200 randomly selected frames, where we selected the vrig subset of HyperNeRF, which contains four scenes.
% The multi-view dataset Neu3D~\cite{li2022neural}  is captured using 15 to 20 static cameras, involves longer durations, and exhibits complex camera motions. 

% Following the previous works~\cite{wu20244d, XXXX}, we extracted the camera poses using SfM from the first frame of each video in the Neu3D~\cite{li2022neural} dataset. We set the rendering resolutions for the D-NeRF~\cite{pumarola2021d}, HyperNeRF~\cite{park2021hypernerf}, and Neu3D~\cite{li2022neural} datasets to 800 × 800, 536 × 900, and 1352 × 1024, respectively.






\subsection{Experiment Protocols}
\noindent\textbf{Datasets.}  We conducted comprehensive experiments on two monocular datasets, D-NeRF~\cite{pumarola2021d} and HyperNeRF~\cite{park2021hypernerf}, and one multi-view dataset, Neu3D~\cite{li2022neural}. Specifically, the monocular dataset, D-NeRF, is a synthetic monocular video dataset specifically designed for monocular settings, where camera poses are generated in a near-random manner for each timestamp. The monocular dataset, HyperNeRF, uses points computed by structure-from-motion (SfM) from 200 randomly selected frames, where we selected the vrig subset comprising four scenes. The multi-view dataset is captured using 15 to 20 static cameras, covers longer durations, and exhibits complex camera motions.
%
The rendering resolutions were set to 800 × 800 for D-NeRF, 536 × 900 for HyperNeRF, and 1352 × 1024 for Neu3D.
\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}

\vspace{-2mm}
\begin{tabular}{lcccc}
\noalign{\hrule height 1pt}
\rowcolor[HTML]{FFFFFF} 
\textbf{Methods} & \textbf{PSNR$\uparrow$} & \textbf{DSSIM$\downarrow$} & \textbf{LPIPS$\downarrow$} & \textbf{Size$\downarrow$} \\
\noalign{\hrule height 1pt}
Hexplane~\cite{cao2023Hexplane}        & 31.71 & \cellcolor{pink}{0.014}  & 0.075      & 200  \\
Kplanes~\cite{fridovich2023k}         & 31.63 & 0.018  &            & 311  \\ \hline
 4DGS~\cite{wu20244d}            & 31.49 & 0.0151 & 0.058      & 38.1 \\
Saro-GS~\cite{yan20244d}         & \cellcolor{pink}{32.03} & \cellcolor{yellow}{0.0142} & \cellcolor{pink}{0.044}      & 385  \\
C-D3DGS~\cite{katsumata2024compact}          & 30.46 & -      & -          & 338  \\
Real-time 4DGS~\cite{yang2023real}   & 32.01 &  \cellcolor{pink}{0.014}  & 0.055      & 6270 \\
% STG\cite{li2024spacetime}              & \cellcolor{pink}{32.04} & 0.0145 & \cellcolor{pink}{0.044}      & 175  \\
Dynamic 3DGS~\cite{luiten2024dynamic}     & 30.46 & 0.019  & 0.099      & 2772 
\\ \hline
Ours (4DGS) high    & 31.54 & 0.0155 & 0.062       & 3.2  \\
Ours (4DGS) mid    & 31.34 & 0.0155 & 0.064       & \cellcolor{yellow}{2.6}  \\
Ours (4DGS) low     & 30.97 & 0.0160  & 0.065       & \cellcolor{pink}{2.3}  \\
Ours (Saro-GS) high & \cellcolor{yellow}{31.93} & 0.0147 & \cellcolor{yellow}{0.045}      & 20.9 \\
Ours (Saro-GS) mid  & 31.73 & 0.0153 & 0.048      & 18.5 \\
Ours (Saro-GS) low  & 31.60  & 0.0154 & 0.047      & 17.0
\\\hline
\noalign{\hrule height 1pt}

\vspace{-1mm}
\end{tabular}
\vspace{-2mm}

\caption{Quantitative comparisons results on Neu3D dataset. The best and second-best results are highlighted in \colorbox{pink}{\textcolor{black}{red}} and \colorbox{yellow!50}{\textcolor{black}{yellow}} cells, respectively. The size values are measured in megabytes (MB). At three distinct storage levels, our 4DGS variant achieves compression ratios of \textbf{$\textbf{11.9}\times$}, \textbf{$\textbf{14.6}\times$}, and \textbf{$\textbf{16.6}\times$} , while our Saro-GS variant achieves compression ratios of \textbf{$\textbf{18.4}\times$},{$\textbf{20.8}\times$},{$\textbf{22.6}\times$}, compared to baseline methods 4DGS and Saro-GS.
}
\label{neu3d}

\end{table}

\noindent\textbf{Evaluation Metric.}
We measure the storage used for 4DGS data using the metric of storage size in megabytes (MB). The quality of the rendered images from the 4DGS methods is evaluated using peak-signal-to-noise ratio (PSNR), perceptual quality measure LPIPS \cite{zhang2018unreasonable}, structural similarity index (SSIM) \cite{wang2004image} and its extensions including structural dissimilarity index measure DSSIM.


\noindent\textbf{Implementation Details.}
Although our 4DGS-CC framework can theoretically be applied to most deformable 3DGS dynamic scene methods, we have chosen to implement it on two representative approaches: 4DGS~\cite{wu20244d} (referred to as Ours (4DGS)) and the latest work SaRO-GS~\cite{yan20244d} (referred to as Ours (SaRO-GS)). Both methods support multi-view and monocular settings.
%
We inherit the hyperparameter configurations (\eg, learning rate for the Gaussian's attitude and the Gaussian deformation field) from~\cite{wu20244d, yan20244d}. To achieve multi-rate compression, we simply use both the codebook size and the user-specific hyperparameter $\lambda$ to adjust storage, denoting the resulting configurations as high, medium, and low storage rates. Specific hyperparameter settings are provided in the supplementary materials. We emphasize that further tuning of the codebook size and $\lambda$, can yield additional storage rate options.
%
We optimized our framework using the Adam optimizer and implemented it in PyTorch with CUDA support. Our experiments based on 4DGS (\ie, Ours (4DGS)) were conducted on an NVIDIA 3090 GPU, while those based on Saro-GS (\ie, Ours (Saro-GS)) were executed on an NVIDIA A100 GPU.


\begin{figure*}
  \centering
    % \fbox{\rule{0pt}{2in} \rule{1\linewidth}{0pt}}
    \includegraphics[width=1\linewidth]{picture/vis.pdf}
    \caption{Visualization comparison between our baseline and our methods  on the ``Flame-steak" scene from the Neu3D dataset. PSNR, LPIPS and the size (MB) of the scene are reported.}
    \label{Vis}
\end{figure*}

\noindent\textbf{Benchmarks.} 
% We compare our 4DGS-CC framework with existing state-of-the-art dynamic scene reconstruction methods.
% We first include NeRF-based dynamic scene methods that incorporate 4D neural voxels, including Hexplane~\cite{cao2023Hexplane}, V4D~\cite{gan2023v4d}, TiNeuVox~\cite{fang2022fast}, and Kplanes~\cite{fridovich2023k}. 
% %
% We also include deformable 3DGS dynamic scene rendering methodology, which are Dynamic 3DGS~\cite{luiten2024dynamic}, C-D3DGS~\cite{katsumata2024compact}, Real-time 4DGS~\cite{yang2023real} along with our baselines Saro-GS\cite{yan20244d}, 4DGS~\cite{wu20244d}.
% %
% It is worth mentioning that, Some deformable 3DGS methods cannot be straightfoward applied for both view setting 
%  (\ie, monocular and multi-view).  For example, XXXX can only be applied in monocular setting but not XXX setting. 
We compare our 4DGS-CC framework with state-of-the-art dynamic scene reconstruction methods. First, we include NeRF-based dynamic scene methods which utilize 4D neural voxels, which are Hexplane~\cite{cao2023Hexplane}, V4D~\cite{gan2023v4d}, TiNeuVox~\cite{fang2022fast}, and Kplanes~\cite{fridovich2023k}. We also include 3DGS dynamic scene rendering approaches, namely, Dynamic 3DGS~\cite{luiten2024dynamic}, C-D3DGS~\cite{katsumata2024compact}, Deformable 3DGS~\cite{yang2024deformable} and Real-time 4DGS~\cite{yang2023real}, along with our baselines Saro-GS~\cite{yan20244d} and 4DGS~\cite{wu20244d}. It is important to note that some methods cannot be straightforwardly applied to both viewing settings (\ie,  monocular and multi-view). For example, Dynamic 3DGS \cite{luiten2024dynamic} is applicable only in a multi-view setting, not in a monocular setting.







% \begin{table}[htbp]
%   \centering
%   \hfill
%   \caption{Neu3D}
%   \begin{minipage}[t]{0.5\textwidth}
%     \centering
%  \begin{tabular}{lllll}
% \begin{tabular}{lllll}
%                  & PSNR  & DSSIM  & LPIPS-alex & Size \\\hline
% Hexplane         & 31.71 & 0.014  & 0.075      & 200  \\
% MixVoxels-X      & 31.73 & 0.015  & 0.064      & 500  \\
% Kplanes          & 31.63 & 0.018  &            & 311  \\ \hline
% 4DGS             & 31.49 & 0.0150 & 0.058      & 38.1 \\
% Saro-GS          & 32.03 & 0.0142 & 0.044      & 385  \\
% C-D3DGS          & 30.46 & -      & -          & 338  \\
% Real-time 4DGS   & 32.01 & 0.014  & 0.055      & 6270 \\
% STG              & 32.04 & 0.0145 & 0.044      & 175  \\
% Dynamic 3DGS     & 30.46 & 0.019  & 0.099      & 2772 \\
% E-3DGS           & 31.20  & 0.0151 & 0.030       & 40.2 \\ \hline
% Our 4DGS high    & 31.54 & 0.0155 & 0.062       & 3.2  \\
% Our 4DGS low     & 30.97 & 0.016  & 0.065       & 2.3  \\
% Our Saro-GS high & 31.93 & 0.0147 & 0.045      & 20.9 \\
% Our Saro-GS low  & 31.60  & 0.0154 & 0.047      & 17
% \\\hline
% \end{tabular}
% \end{tabular}
%   \end{minipage}
% \end{table}



% \begin{table}[htbp]
%   \centering
%   \hfill
%   \caption{Hypernerf}
%   \begin{minipage}[t]{0.5\textwidth}
%     \centering
%  \begin{tabular}{llllll}
%                 & PSNR  & SSIM  & LPIPS-v & Size 
% \\\hline
% 4DGS            & 25.17 & 0.685 & 0.33  & 65   \\
% C-D3DGS         & 25.6  & -     & -     & 720  \\
% SC-GS           & 21.19 & 0.575 & 0.31  & 232  \\
% Deformable 3DGS & 22.72 & 0.616 & 0.35  & 138  \\ \hline
% Our 4DGS high   & 25.21 & 0.683 & 0.34  & 5    \\
% Our 4DGS low    & 25.11 & 0.678 & 0.34  & 3.8 \\\hline
% \end{tabular}
%   \end{minipage}
  
% \end{table}



\begin{table}[h]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.3}

\vspace{-2mm}
\begin{tabular}{lcccc}
\noalign{\hrule height 1pt}
\rowcolor[HTML]{FFFFFF} 
\textbf{Methods} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{Size$\downarrow$} \\
\noalign{\hrule height 1pt}
TiNeuVox-B~\cite{fang2022fast} & 24.3 & - & - & 48  \\
V4D~\cite{gan2023v4d}        & 24.8 & - & - & 377 \\ \hline
4DGS~\cite{wu20244d}            & 25.17 & \cellcolor{pink}{0.685} & \cellcolor{pink}{0.33}  & 65   \\
C-D3DGS~\cite{luiten2024dynamic}         & \cellcolor{pink}25.6  & -     & -     & 720  \\
Deformable 3DGS~\cite{yang2024deformable} & 22.72 & 0.616 & 0.35  & 138  \\ \hline
Ours (4DGS) high   & \cellcolor{yellow}{25.21} & \cellcolor{yellow}{0.683} & \cellcolor{yellow}{0.34}  & 5.0    \\
Ours (4DGS) mid     & 25.18 & 0.682 & 0.34  & \cellcolor{yellow}4.4 \\
Ours (4DGS) low    & 25.11 & 0.678 & 0.35  & \cellcolor{pink}{3.8} \\
\noalign{\hrule height 1pt}
\end{tabular}
\caption{Quantitative comparisons result on the HyperNeRF dataset. The best and second-best results are highlighted in \colorbox{pink}{\textcolor{black}{red}} and \colorbox{yellow!50}{\textcolor{black}{yellow}} cells, respectively. The size values are measured in megabytes (MB). At three distinct storage levels, our 4DGS variant achieves compression ratios of {$\textbf{13.0}\times$}, {$\textbf{14.7}\times$} and {$\textbf{17.8}\times$} compared to baseline methods 4DGS.
}
\label{hypernerf}
\vspace{-2mm}
\end{table}

\subsection{Experimental Results}
We present quantitative comparison results on the D-NeRF~\cite{pumarola2021d}, Neu3D~\cite{li2022neural}, and HyperNeRF datasets~\cite{park2021hypernerf} in Table \ref{d-nerf}, Table \ref{neu3d}, and Table \ref{hypernerf}, respectively. Notably, our 4DGS-based variant with a high storage-rate setting (\ie, Ours (4DGS) high) achieves even better reconstruction performance than the baseline 4DGS method, while obtaining compression ratios of 12.3×, 11.9×, and 13.0× on the D-NeRF~\cite{pumarola2021d}, Neu3D~\cite{li2022neural}, and HyperNeRF datasets~\cite{park2021hypernerf} datasets, respectively.

Similarly, our Saro-GS-based variant with a high storage-rate setting (\ie, Ours (Saro-GS) high) achieves comparable reconstruction performance to the baseline Saro-GS method, while delivering compression ratios of 8.9× and 18.4× on the D-NeRF~\cite{pumarola2021d} and Neu3D~\cite{li2022neural} datasets. Additionally, our Saro-GS-based variant with a low storage-rate setting (\ie, Ours (Saro-GS) low) achieves compression ratios of up to 11.3× and 22.6× on the D-NeRF~\cite{pumarola2021d} and Neu3D~\cite{li2022neural} datasets, respectively, with only a slight reduction in reconstruction quality. This indicates that our methods accommodate a wide range of compression scenarios, from low to high qualit, to meet various application needs.


% On synthetic dataset D-NeRF, compared to our baseline method~\cite{wu20244d},~\cite{yan20244d}, our approach consistently achieves comparable or even higher reconstruction quality at our high rate while achieved compression ratios of $11.8\times$ and $10\times$, respectively. 
% At the same time, our method outperforms other 3DGS-based and NeRF-based methods in terms of both PSNR and storage. 
% On the real-world multiview Neu3D dataset~\cite{li2022neural}, our approach consistently achieves comparable or even higher reconstruction quality at our high rate while achieved compression ratios of $11.9\times$ and $18.4\times$, respectively. 
% At the same time, our method outperforms other 3DGS-based and NeRF-based methods in terms of storage. 
% On the HyperNeRF~\cite{park2021hypernerf} dataset,we only report the results of Our 4DGS-based variant (\ie,Ours (4DGS)) , as Saro-GS~\cite{yan20244d} did not provide its results on HyperNeRF. Our approach consistently achieves comparable or even higher reconstruction quality at our high rate while achieved compression ratios of $13\times$. At the same time, our method outperforms other 3DGS-based and NeRF-based methods in storage. 
% Compared to other baselines, our results are competitive, while requiring much less storage. Even compared to NeRF-based methods, our storage performance shows a significant advantage. The RD curves for different datasets are provided in Figure.

% We offer qualitative comparisons for the xxx scenes.We demonstrate that our method achieves rendering results comparable to the uncompressed version in terms of detail preservation.

\subsection{Ablation Study}

\textbf{Effectiveness of Individual Compression Components.} We conduct extensive ablation studies on our 4DGS-based method (\ie, Ours (4DGS)) to evaluate the impact of compressing two components, which are Canonical Gaussians and 4D Neural Voxels, on the HyperNeRF dataset. Specifically, we examine two variants: Ours (4DGS) w/o CG, which compresses only the 4D Neural Voxels, and Ours (4DGS) w/o NV, which compresses only the Canonical Gaussians. As shown in Fig.~\ref{fig:ab1}, compressing either component alone yields significant storage savings compared to the baseline 4DGS. Moreover, combining these two components in our full 4DGS-based method (\ie, Ours (4DGS)) achieves further storage reductions of 89.0\% and 86.2\% compared to the variants, Ours (4DGS) w/o CG and Ours (4DGS) w/o NV, respectively. This observation indicates that simultaneously compressing both components in a dual-compression fashion is highly beneficial.

\begin{figure}
  \centering
   \includegraphics[width=0.85\linewidth]{picture/aba.pdf}
    \vspace{-2mm}
   \caption{Ablation study of two compression components on the HyperNeRF dataset.
   (1) \textbf{4DGS:} Our baseline 4DGS.
   (2) \textbf{Ours (4DGS) w/o CG:} Our method based on 4DGS without the compression of Canonical Gaussian.
   (3) \textbf{Ours (4DGS) w/o NV:} Our method based on 4DGS without the compression of Neural Voxel.
   (4) \textbf{Ours (4DGS):} Our method based on 4DGS.}
    \label{fig:ab1}
\end{figure}
\begin{figure}
  \centering
   \includegraphics[width=0.85\linewidth]{picture/abnv.pdf}
    \vspace{-2mm}
   \caption{Ablation study of components within NVCC strategy on the HyperNeRF dataset 
   (1) \textbf{Ours (4DGS) w/o NVCC:} Our method based on 4DGS without using NVCC.
   (2) \textbf{Ours (4DGS) w/o SP:} Our method based on 4DGS without using spatial prior when performing NVCC.
   (3) \textbf{Ours (4DGS) w/o HF:} Our method based on 4DGS without updating the temporal priors with the hidden feature when performing NVCC.
   (4) \textbf{Ours (4DGS):} Our method based on 4DGS.}
    \label{fig:ab2}
    \vspace{-4mm}
\end{figure}

\textbf{Effectiveness of each compoents in NVCC.}
We also conduct ablation studies on our 4DGS-based method (\ie, Ours (4DGS)) on the HyperNeRF dataset to evaluate the effectiveness of each individual component within NVCC when losslessly compressing the quantized features of 4D Neural Voxels. Specifically, we examine three variants: the first variant (\ie, Ours (4DGS) w/o SP) uses only temporal priors, omitting the spatial prior; the second variant (\ie Ours (4DGS) w/o HF) does not employ the hidden feature updating mechanism for temporal priors; and the third variant (Ours (4DGS) w/o NVCC) does not apply NVCC for further lossless compression of the quantized 4D Neural Voxels. As shown in Fig.~\ref{NVCC}, both the Ours (4DGS) w/o HF and Ours (4DGS) w/o SP variants, which incorporate NVCC components, achieve significant storage savings compared to the variant that does not use NVCC, saving 63\% and 65\% respectively. Furthermore, combining all components leads to further performance enhancements. This observation underscores the importance of these components in the lossless compression of 4D Neural Voxels.

\textbf{Effectiveness of VQCC.} We further conduct ablation studies on HyperNeRF~\cite{park2021hypernerf} dataset for our 4DGS-based method (\ie, Ours (4DGS)) to evaluate the effectiveness of VQCC, which losslessly compresses the quantized codebook. In our experiments, we directly store the quantized codebook when compressing the Canonical Gaussians without applying VQCC (\ie, Ours (4DGS) w/o VQCC). It is observed that this variant introduces an extra storage cost, demonstrating the importance of effective lossless compression of the codebook.

\begin{figure}
  \centering
   \includegraphics[width=0.85\linewidth]{picture/abc.pdf}
    \vspace{-2mm}
   \caption{Ablation study of VQCC strategy on the HyperNeRF dataset.
   (1) \textbf{Ours (4DGS) w/o VQCC:} Our method based on 4DGS without using VQCC to further losslessly compress the codebook.
   (2) \textbf{Ours (4DGS):} Our method based on 4DGS.}
   
    \label{fig:ab3}
\end{figure}
\subsection{Visualization}
Our visualization results are displayed in Fig. \ref{Vis}, showing rendered outputs for the ``Flame-steak" scene from the Neu3D dataset~\cite{li2022neural} dataset.
It can be observed that even under high compression ratios, our approach preserves the rendering fidelity of the original method in challenging regions. For example, in the ``Flame-steak" scene, both our method and Saro-GS~\cite{yan20244d} capture details of the face of the dog.The maintained or improved fidelity metrics (\eg, PSNR and LPIPS) further demonstrate the superior quality of our method.

% Regarding the MLP-based context module, we analyze the rationality of the context design, as shown in the results. We first test a design without level context, proving the effectiveness of the level context module. Additionally, to demonstrate the temporal attention-based context design, we test the effects of using $n_{tem} = \{n_{v_1 - 1, v_2}\}$ and $n_{tem} = \{n_{v_1 - 1, v_2}, n_{v_1 - 2, v_2}, \dots, n_{v_1 - 5, v_2}\}$ as contexts for $n_{v_1, v_2}$. Results show that our method outperforms simpler designs using only the previous one or five timestamps.We believe that the reason for the poor performance when using only one timestamps is primarily due to the failure to fully leverage temporal correlations. For instance, it cannot make probabilistic predictions by capturing the trends across multiple timestamps. On the other hand, the reason for the suboptimal performance when using five timestamps is likely due to the limited size of the context model. Since the context model is designed as a tiny MLP, the complexity of five timestamps makes it difficult for the model to fit effectively.


==> ICCV2025-Author-Kit/6_conclusion.tex <==
\section{Conclusion}
In this work, we propose the first neural contextual coding framework for compressing 4DGS data. Our approach builds on the deformable 3DGS framework and performs a lossy-lossless compression of two key components: Canonical Gaussians and 4D Neural Voxels. After applying lossy compression to these components, we further enhance lossless compression by introducing two innovative neural contextual coding strategies, VQCC and NVCC to entropy coding.
%
Extensive experiments demonstrate that our framework achieves significant storage reductions compared to other 4DGS methodologies while enabling variable-rate compression. We believe this work bridges the gap between 4DGS and data compression research, paving the way for broader future investigations.

\noindent\textbf{Limitations and Future Work.} Currently, our 4DGS-CC framework is implemented only with deformable 3DGS approaches that utilize Hexplane 4D Neural Voxels in the deformation field. In future work, we plan to extend our framework to a broader range of deformable 3DGS methods, including those that employ 4D Hash Grids in the deformation field, thereby enhancing its general applicability.

==> ICCV2025-Author-Kit/sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> ICCV2025-Author-Kit/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> ICCV2025-Author-Kit/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> ICCV2025-Author-Kit/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> mydef.tex <==
% % \usepackage{amsmath}
% \usepackage{etoolbox}
% \usepackage{bm}
% \usepackage{amsthm}%
% %\usepackage{mathtools}%
% % \usepackage{algorithm}%
% % \usepackage{algorithmic}%
% \usepackage{subfigure}%

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \newtheorem{deftn}{Definition}
% \newtheorem{thm}{Theorem}
% \newtheorem{prop}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{remark}{Remark}

\newcommand{\MyMapTemplatePrefixc}[4]{\expandafter#1\csname#3#4\endcsname{#2{#4}}} % it remembles a template: \#3#4 --> #2{#4}
\forcsvlist{\MyMapTemplatePrefixc {\def} {\mathcal}{c}} {A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}  % e.g., \cA --> \mathcal{A}

\newcommand{\MyMapTemplatePrefixtb}[5]{\expandafter#1\csname#4#5\endcsname{#2{#3{#5}}}} % it remembles a template: \#3#4 --> #2{#4}
\forcsvlist{\MyMapTemplatePrefixtb {\def} {\tilde}{\mathbf}{t}} {A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}  % e.g., \tA --> \tilde{A}
\forcsvlist{\MyMapTemplatePrefixtb {\def} {\tilde}{\mathbf}{t}} {0,1,a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,u,v,w,x,y,z}  % e.g., \ta --> \tilde{a}

\newcommand{\MyMapTemplateNoPrefix}[3]{\expandafter#1\csname#3\endcsname{#2{#3}}}
\forcsvlist{\MyMapTemplateNoPrefix {\def} {\mathbf} } {0,1,a,b,c,d,e, f, g, h, i, j, k, l, m, n, o, p, q, r, u, v, w, x, y, z} % e.g., \a --> \mathbf{a}
\forcsvlist{\MyMapTemplateNoPrefix {\def} {\mathbf} } {A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}  % e.g., \A --> \mathcal{A}

\def\ba{\bm{\alpha}}
\def\bb{\bm{\beta}}
\def\bd{\bm{\delta}}
\def\bt{\bm{\theta}}
\def\bz{\bm{\zeta}}

\def\bP{\bm{\Phi}}
\def\bQ{\bm{\Psi}}
\def\bS{\bm{\Sigma}}

\def\bbR{{\mathbb R}}
\def\bbE{{\mathbb E}}

\def\tr{\mbox{tr}}
\def\Pr{{P}}

\def\etal{\emph{et al.}\@\xspace}
\def\ie{\emph{i.e.}\@\xspace}
\def\eg{\emph{e.g.}\@\xspace}
\def\resp{\emph{resp.}\@\xspace}

\definecolor{rowblue}{RGB}{220,230,240}


==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
